Efficient Strategy Synthesis for MDPs with Resource Constraints

We consider qualitative strategy synthesis for the formalism called consumption Markov decision processes. This formalism can model dynamics of an agents that operates under resource constraints in a stochastic environment. The presented algorithms work in time polynomial with respect to the representation of the model and they synthesize strategies ensuring that a given set of goal states will be reached (once or infinitely many times) with probability 1 without resource exhaustion. In particular, when the amount of resource becomes too low to safely continue in the mission, the strategy changes course of the agent towards one of a designated set of reload states where the agent replenishes the resource to full capacity; with sufficient amount of resource, the agent attempts to fulfill the mission again. We also present two heuristics that attempt to reduce expected time that the agent needs to fulfill the given mission, a parameter important in practical planning. The presented algorithms were implemented and numerical examples demonstrate (i) the effectiveness (in terms of computation time) of the planning approach based on consumption Markov decision processes and (ii) the positive impact of the two heuristics on planning in a realistic example.

==> labels.tex <==
\section{Labeled CMDPs}
\fixme

\smallskip \noindent%
\textbf{Labeled CMDPs, Deterministic Büchi Automata and LTL.} %
The algorithm in~\cite{Blaetal20} synthesizes a resource-constrained strategy
for almost-sure satisfaction of a Büchi objective, where the accepting states
have to be explicitly specified. \FiMDP{} now fully supports CMDPs with states
labeled by sets of atomic propositions. Given such a labeled CMDP $\mdp$ and a
deterministic Büchi automaton $\automaton$ over the same atomic propositions,
\FiMDP{} can synthesize a resource-aware strategy that produces (for a suitable
initial level of resource) runs whose labeling is almost surely accepted by
$\automaton$. To achieve this, \FiMDP{} follows the classical approach of
constructing and analyzing the \emph{product} $\mdp\otimes\automaton$ via the
standard \emph{synchronous parallel composition} technique~\cite{BaiKat08}.

Obviously, the counter strategy synthesized for $\mdp \otimes \automaton$
operates correctly only on this product, which might be impractical. For the
convenience of users, \FiMDP{} provides a capability to synthesize a counter
strategy which stores $\automaton$ in its memory. This means, the strategy
tracks in memory both the resource level (using a counter) and the progress in
$\automaton$, and base its decisions based on the current state, the current
resource level, and the current state of the automaton. As a result, the users
can run these strategies on their original model. Another advantage of these
strategies is that the potentially large object for $\mdp\otimes\automaton$ can
be discarded from memory right after the analysis.

The product-based approach extends naturally to the recurrence fragment of linear
temporal logic. Given a formula $\ltlform$ of this fragment and a labeled CMDP
$\mdp$, \FiMDP{} can compute the values $\minlev_\ltlform$ and synthesize a strategy $\sigma$, which operates on $\mdp$ and which has the following properties:

\fixme{} probability measure defined differently in the two papers
\begin{enumerate}%[a)]
\item for all $ t\in \Nset $, $ \probm{\sigma}{\fixme}(r_t < 0 \mid s_0 = s, r_0 = \minlev_\ltlform(s)) = 0$; and
\item $ \probm{\sigma}{\fixme}(\ltlform \text{ is satisfied by the sample run}  \mid s_0 = s, r_0 = \minlev_\ltlform(s) )  = 1$.
\end{enumerate}

This capability is justified by the fact that each formula of the recurrence
fragment can be translated to an equivalent DBA~\cite{manna.90.podc}. \FiMDP{}
uses the \Spot{} library~\cite{duret.16.atva} for this translation and then
employs the product approach described above. The user requires just one line of
code with \FiMDP{} to run this pipeline and get a strategy without ever being
exposed to the product construction.


==> tikzlibrarycmdps.code.tex <==
%oo\tikzstyle{target}=[fill=blue!15]
%\tikzstyle{reload}=[accepting]

\tikzset{state/.append style={fill=blue!4}}
\tikzstyle{target}=[fill=green!70!black!25]
\tikzstyle{reload}=[accepting]

% Probability labels
\tikzstyle{prob}=[
  color=black!50,
  outer sep=-2pt,
  pos=.8,
]

% Consumption labels
\tikzstyle{cons} = [
  execute at begin node = {$[$},%
  execute at end node = {$]$},
  outer sep=0pt,
  pos=.5,
]

\tikzstyle{shifted below} = [
  below,  outer sep=15pt,
]

% Value boxes
\tikzstyle{valbox} = [
  rounded corners=2pt,
  shifted below,
  inner sep=.5pt,
  draw,
  font=\footnotesize,
  minimum size=1em,
]

\tikzset{
  objective/.style = {
    label={[label position=north, anchor=south, below,
    xshift=0pt, yshift=-4pt,
    fill=white, scale=.5,
    draw, rounded corners=1pt, very thin]#1}
  },
  obj prob/.style = {
    label={[label position=south, anchor=north, above,
    xshift=0pt, yshift=4pt,
    fill=white, scale=.5,
    draw, rounded corners=1pt, very thin]#1}
  },
  nonreloading/.style = {
    objective=$\nonreloading$,
    fill=orange!15,
  },
  safety/.style = {
    objective=$\safety$,
    fill=blue!15,
  },
  pos reach/.style = {
    objective=$\reachability$,
    obj prob=${}>0$,
    fill=green!70!black!20,
  },
  as reach/.style = {
    objective=$\reachability$,
    obj prob=$\as$,
    fill=green!70!black!20,
  }
}

\tikzstyle{capacity} = [
  rounded corners,
  draw,
  fill=yellow!40,
]

==> tikzlibrarygridworld.code.tex <==
\usepackage{xcolor}

\usetikzlibrary{arrows.meta}

\definecolor{background}{rgb}{0.85,1.0,1.0}
\definecolor{agent}{rgb}{0.42,0.42,0.42}

\tikzstyle{action edge} = [thick,shorten >=1pt,>={Stealth[round]}]
\tikzstyle{side effect} = [gray, shorten >=4pt, looseness=\loose, green!60!black!40]
\tikzstyle{main} = [shorten >=-4pt, very thick, green!60!black]

\tikzstyle{agent} = [minimum size=15pt, rounded corners, draw=agent,fill=agent]
\tikzstyle{action name} = [font={\scriptsize\sffamily}, align=center, scale=.7]
\tikzstyle{gridworld} = [gray, ultra thin]

%\tikzstyle{reload} = []

\def\loose{.7}

==> tikzlibrarymyautomata.code.tex <==
% Automata stuff
\usetikzlibrary{automata}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{bending}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{matrix}
\usetikzlibrary{shapes}

\def\accsize{6pt}

\tikzset{
  >={Stealth[round,bend]},
}

\tikzstyle{automaton}=[
  % Use nice arrows that do not touch their destination.
  semithick,shorten >=1pt,>={Stealth[round,bend]},
  % Encourage a common distance between all states.
  node distance=1.7cm,
  % Disable the "start" text in front of the initial arrow.
  initial text=,
  % Allows to use scale to scale the figure
%  transform shape,
  % Reduce the size of the hidden node at the beginning of the initial arrow.
  every initial by arrow/.style={every node/.style={inner sep=0pt}},
  % Encourage a common size of all states that is smaller than the default.
  every state/.style={
    align=center,
    fill=white,
    minimum size=6mm,
    inner sep=0pt,
  },%
]

\tikzstyle{smallautomaton}=[
  automaton,
  node distance=8mm,
  every state/.style={minimum size=4mm,fill=white,inner sep=1pt}
]

\tikzstyle{mediumautomaton}=[
  automaton,
  node distance=1cm,
  every state/.style={minimum size=5mm,fill=white,inner sep=2pt}
]

\tikzstyle{cstate}=[state,rounded rectangle,text width=,]

% This is used for runs vizualization
\tikzstyle{dot}=[fill=black,circle,minimum size=4pt,inner sep=0]

\makeatletter
\tikzoption{initial angle}{\tikzaddafternodepathoption{\def\tikz@initial@angle{#1}}}
\makeatother

% pass "initial overlay" as a parameter to the tikz figure if you want
% to initial arrow to be ignored from the computation of the figure
% box.  This might be needed for better caption centering.
\tikzstyle{initial overlay}=[every initial by arrow/.append style={overlay}]

\tikzstyle{unreachable} = [densely dotted]

% % % Usage: \node[acclabel]{label\strut}
% The command \strut makes all labels have the same height.
\tikzstyle{acclabel} = [
  fill=yellow!20,
  rounded corners=3pt,
  draw=black,
  inner ysep=0pt,
  inner xsep=3pt,
]
\tikzstyle{ltllabel} = [acclabel,fill=darkgreen!20]

\tikzstyle{namelabel} = [
  execute at begin node = {$($},%
  execute at end node = {$)$}
]

\tikzstyle{matrix of states} = [
matrix of nodes,
every node/.style={state},
column sep=.8cm,
row sep=.8cm,
execute at empty cell={
  \node[transparent,name=
    \tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn]{};]},
]

% Acceptance sets are displayed as small circles with white
% sans-serif number.  The default color is light blue. Can be
% changed by collacc styles.  Use anchor=center to ignore the
% predefined anchor on edges like "loop above" or "loop left"
% or when using path[auto].
\tikzstyle{accset}=[
  circle,inner sep=.9pt,
  draw=none, %draw=white,
  solid,
  collacc0, text=white,
  thin,
  anchor=center,
  font=\bfseries\tiny, %\sffamily
  minimum size={\accsize},
]
% Acceptance set as square
\tikzstyle{accsquare}=[accset,rectangle,inner sep=1.9pt,rounded corners=0pt]

% % % Colors % % %
\tikzset{
  collacc0/.style={fill=blue!50!cyan},
  collacc1/.style={fill=orange!90!black},
  collacc2/.style={fill=green!70!black},
  collacc3/.style={fill=red!80!black},
  collacc4/.style={fill=magenta},
  collacc5/.style={fill=blue!50!black},
}


% The key /sacc/where is used to determine where the acc marks on
% states should be placed using the sacc/derived keys
% The default value is center
% It has to be used in scopes, does not work inside nodes
\pgfkeyssetvalue{/sacc/where}{center}
\tikzset{
  sacc where/.code={
    \pgfkeyssetvalue{/sacc/where}{#1}
  }
}

% % % Labels and marks of automata % % %
\tikzset{
  % Labels of edges that have some acceptance mark. Shifts label
  % further from the edge to avoid ugly clash with the mark.
  % Usage:
  %   (n1) edge pic[pos=.3,left]{l=LABEL}
  l/.pic={\node[outer sep=3pt] {#1};},%
  % A colored mark with number inside. Use acc for a small circle and
  % accsq for a small square.
  % Usage:
  %   (n1) edge pic[pos=.3]{acc=ACC_ID}
  % collaccACC_ID must be defined
  acc/.pic={\node[accset,collacc#1]{#1};},%
  accsq/.pic={\node[accsquare,collacc#1]{#1};},%
  % No number inside the bullets
  eacc/.pic={\node[accset,collacc#1]{\emptyacc};},%
  eaccsq/.pic={\node[accsquare,collacc#1]{\emptyacc};},%
  % State labels on north east
  sacc/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {acc=#1}}
  },
  saccsq/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {accsq=#1}}
  },
  esacc/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {eacc=#1}}
  },
%  esacc/.style 2 args = {
%    append after command=
%      {pic[#2] at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {eacc=#1}}
%  },
  esaccsq/.style = {
    append after command=
      {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {eaccsq=#1}}
  },
  % Easy typesetting of colored accepting marks with custom labels.
  % Usage:
  %   (n1) edge pic[pos=.3]{acc={COLOR_ID}{LABEL}}
  % collaccCOLOR_ID must be defined
  pics/cacc/.style 2 args={%
    code={\node[accset,collacc#1]{#2};}%
  },%
  pics/caccsq/.style 2 args={%
      code={\node[accsquare,collacc#1]{#2};}%
    },%
  csacc/.style 2 args = {%
      append after command=%
        {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {cacc={#1}{#2}}}%
  },%
  csaccsq/.style 2 args = {%
      append after command=%
        {pic at (\tikzlastnode.\pgfkeysvalueof{/sacc/where}) {caccsq={#1}{#2}}}%
  },%
}

% Macros for colored acceptance marks used in text. Usage:
% \tacc{COLOR_ID}{LABEL}
\def\markbaseline{-.37em}
\def\tacc#1{\tikz[baseline=\markbaseline]\pic{acc=#1};\xspace}
\def\tcacc#1#2{\tikz[baseline=\markbaseline]\pic{cacc={#1}{#2}};\xspace}
\def\taccsq#1{\tikz[baseline=\markbaseline]\pic{accsq=#1};\xspace}
\def\tcaccsq#1#2{\tikz[baseline=\markbaseline]\pic{caccsq={#1}{#2}};\xspace}

% % % some predefined marks with no number inside
\def\emptyacc{\phantom{0}}
\def\gm{\tcacc{2}{\emptyacc}}
\def\om{\tcacc{1}{\emptyacc}}
\def\bm{\tcacc{0}{\emptyacc}}
\def\bsq{\tcaccsq{0}{\emptyacc}}
\def\rsq{\tcaccsq{3}{\emptyacc}}

\def\minimark#1{
\def\emptyacc{}
\def\accsize{4pt}
#1
}

